Energy versus Output Quality of Non-volatile Writes in Intermittent Computing

We explore how to improve the energy performance of battery-less Internet of Things (IoT) devices at the cost of a reduction in the quality of the output. Battery-less IoT devices are extremely resource-constrained energy-harvesting devices. Due to erratic energy patterns from the ambient, their executions become intermittent; periods of active computation are interleaved by periods of recharging small energy buffers. To cross periods of energy unavailability, a device persists application and system state onto Non-Volatile Memory (NVM) in anticipation of energy failures. We purposely control the energy invested in these operations, representing a major energy overhead, when using Spin-Transfer Torque Magnetic Random-Access Memory (STT-MRAM) as NVM. As a result, we abate the corresponding overhead, yet introduce write errors. Based on 1.9+ trillion experimental data points, we illustrate whether this is a gamble worth taking, when, and where. We measure the energy consumption and quality of output obtained from the execution of nine diverse benchmarks on top of seven different platforms. Our results allow us to draw three key observations: i) the trade-off between energy saving and reduction of output quality is program-specific; ii) the same trade-off is a function of a platform's specific compute efficiency and power figures; and iii) data encoding and input size impact a program's resilience to errors. As a paradigmatic example, we reveal cases where we achieve up to 50% reduction in energy consumption with negligible effects on output quality, as opposed to settings where a minimal energy gain causes drastic drops in output quality.

==> Sezioni/Outline.tex <==
% \vspace{-30pt}
% \begin{enumerate}[label={\textbf{\arabic*.}}, left=0pt, align=left, itemindent=*]
%     \item Introduction
%     \item Background
%         \begin{enumerate}[label={\textbf{2.\arabic*.}}, align=left, left=0pt, itemindent=*]
%             \item Intermittent Computing
%                 \begin{itemize}
%                     \item Emphasize the difference between intermittent and continuous execution.
%                     \item Introduce the state persistence routine as an overhead affecting system performance.
%                     \item The addressed problem in this work is the reduction of this overhead.
%                 \end{itemize}
%             \item STT-MRAM
%                 \begin{itemize}
%                     \item Outlook on STT-MRAM, comparing it to other NVMs.
%                     \item Highlight why it is a promising choice for battery-less devices.
%                     \item Introduce its stochastic writing property.
%                     \item Write Approximation:
%                         \begin{itemize}
%                             \item Exploit stochastic switching for an approximation technique by manipulating the write current.
%                             \item Demonstrate how Write Error Rate (WER) changes with the write current.
%                         \end{itemize}
%                 \end{itemize}
%             \item Approximate Computing
%                 \begin{itemize}
%                     \item Introduce concepts of approximate computing.
%                     \item Provide an example, like  with a correct image and its approximate counterpart.
%                 \end{itemize}
%         \end{enumerate}
%     \item Approximate Intermittent Computing: STT-MRAM
%         \begin{itemize}
%             \item Describe the use of STT-MRAM with approximated writes as \ac{NVM} for the state persistence operation in an intermittent computing system.
%             \item Include a plot of the framework, highlighting knobs and results.
%             \item Discuss the advantages of approximated writes.
%             \item Explain the disadvantages of having faulty bits in the persisted state.
%             \item Conclude the section by defining the problem of quantifying the trade-off between energy savings and quality reduction.
%         \end{itemize}
%     \item Evaluation
%         \begin{enumerate}[label={\textbf{4.\arabic*.}}, align=left, left=0pt, itemindent=*]
%             \item Target Platforms
%                 \begin{itemize}
%                     \item Describe different hardware platforms used for evaluation.
%                     \item Explain why a multi-capacitor system is used for STM.
%                 \end{itemize}
%             \item Benchmarks
%                 \begin{itemize}
%                     \item Show selected benchmarks for evaluation.
%                     \item Explain the reason for choosing each benchmark.
%                     \item Justify the transition from general benchmarks (Mibench2) to neural networks.
%                 \end{itemize}
%             \item Evaluation Methodology
%                 \begin{itemize}
%                     \item Describe the framework built to generate results.
%                     \item Include emulators, benchmarks, and energy consumption calculation for STM and MSP430 MCUs.
%                     \item Explain the checkpointing strategy for DNNs.
%                 \end{itemize}
%             \item Results
%                 \begin{itemize}
%                     \item Present and discuss obtained results.
%                     \item Start with conclusions derived from experiments and explore observations leading to these conclusions.
%                     \item Keep conclusions general and benchmark-agnostic.
%                 \end{itemize}
%         \end{enumerate}
%     \item Conclusion
%         \begin{enumerate}[label={\textbf{5.\arabic*.}}, align=left, left=0pt, itemindent=*]
%             \item Summarize key contributions and implications of the research.
%             \item Mention limitations and suggest future work.
%         \end{enumerate}
% \end{enumerate}

